MeetMap: Real-Time Collaborative Dialogue Mapping with LLMs in Online Meetings

Video meeting platforms display conversations linearly through transcripts or summaries. However, ideas during a meeting do not emerge linearly. We leverage LLMs to create dialogue maps in real time to help people visually structure and connect ideas. Balancing the need to reduce the cognitive load on users during the conversation while giving them sufficient control when using AI, we explore two system variants that encompass different levels of AI assistance. In Human-Map, AI generates summaries of conversations as nodes, and users create dialogue maps with the nodes. In AI-Map, AI produces dialogue maps where users can make edits. We ran a within-subject experiment with ten pairs of users, comparing the two MeetMap variants and a baseline. Users preferred MeetMap over traditional methods for taking notes, which aligned better with their mental models of conversations. Users liked the ease of use for AI-Map due to the low effort demands and appreciated the hands-on opportunity in Human-Map for sense-making.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> references_with_notes.tex <==

\section{Related Work}

\subsection{Information Organization and Sense-making to Support Synchronous Group Meetings}

\textcolor{red}{more psychology-leaning items; e.g. what are general issues folks have in meetings (challenges people faced in synchronous group meetings; hard to make sense of chronological information, cognitive load for listening, thinking, and talking at the same time, the common ground theory, etc. PLUS some theories and techniques to help sense-making during synchronous meetings. e.g, facilitation method in CSCL/CSCW (computer supported collab work), designated turn-taking, collaborative note-taking, understanding check}

Participant engagement is crucial to the success of team meetings, as groups working together are able to develop original and feasible ideas more so than individuals \cite{kohnBuildingIdeasOthers2011}. Yet synchronous meetings come with a set of challenges to participants including increased cognitive load and screen fatigue \cite{karl2021virtual}. There are several reasons for challenges like these to arise, including badly structured meetings and the way in which interactions between participants can feel unnatural through virtual meetings \cite{karl2021virtual}. \textcolor{red}{want to make the case that COMMUNICATION can ease cognitive load, and that it can be achieved through visualization of the conversation trajectory}
The adverse effects of obstacles such as cognitive overload can be diminished by an increase in communication \cite{fussellCoordinationOverloadTeam1998}, \textcolor{blue}{since participants do not have go out of their way to understand what the group's status is; in other words, the process of sensemaking and building mutual understanding is a continuous and speedy process in lieue of high-volume and clear communication between participants}. 
\textcolor{blue}{We derive the conclusion that teams with participants experiencing a lower cognitive load will be able to coordinate better}
Meeting success can be predicted by several factors, including focused discussion of meeting content \cite{fussellCoordinationOverloadTeam1998} and the success of participants to build mutual understanding between one another \cite{kecskesActivatingSeekingCreating2009}. Building mutual understanding is a result of individual and group-level sensemaking, and sensemaking is a process that spans across a conversation on both high-level attributes such as general meeting topics as well as granular-level utterances. Encouraging sensemaking and building mutual understanding can be accomplished using supplementary meeting tools and software; specifically, visual cues have been shown to encourage engagement and improve team performance on group tasks \cite{yuExploringHowWorkspace2022}, \cite{liuConsensUsSupportingMultiCriteria2018}, \cite{valkIdeationCompassSupporting2022} and visual information about the conversation at hand can reduce participants' cognitive load by creating ``external memory`` in a user's periphery \cite{kirshenbaum2021traces}, \cite{Pedersen1997AROMAAR}.

\cite{fussellCoordinationOverloadTeam1998} -- communication tactics in meetings that allow for participants to not be overloaded; team coordination + what tools they used predicts success
    - synchronous communication > async comm in terms of overload
    - discussion of the actual content at hand rather than team processes (e.g. logistics) was more of a predictor of success
    - more communication --> less cognitive overload 
\cite{hou2011analyzing} -- case study analysis of knowledge construction in synchronous IM discussions (student groups)
    - social knowledge construction is mainly done using sharing + comparing (as opposed to e.g. negotiation or working through conflict)
    - off-topic discussions more likely in synchronous discussions than async
    - the highest-quality discussions exhibited more coordination
    - high coordination is related to joint decision making rather than individuals making their own ways
\cite{karl2021virtual} -- lays out issues w/ work meetings during the pandemics
    - common issues of being on video-conference calls all the time: information overload from staring at screen, communication thru virtual mtg is less natural and more tiring
    - badly structured meetings --> participants disengaged 
\cite{kecskesActivatingSeekingCreating2009} -- more of psychology theory on how meeting participants get along
    - mutual understanding is a sequential process that is built up from interactions between individuals; this is especially important for initial meetings between a team where the participants might not be as familiar with each other 
    - sensemaking can be a process of collecting info from across the conversation 
\cite{kirshenbaum2021traces} -- they analyze the effectiveness of a tool SAGE2 that allows users to share content on a canvas in parallel with the main presenter
    - advantages is that this is a source for 'external memory' which can reduce cognitive load
\cite{kohnBuildingIdeasOthers2011} -- basically just that groups come up w more novel + feasible ideas than individuals
\cite{yuExploringHowWorkspace2022} -- insights into collaborative knowledge sharing in meetings
    - this is very similar to MeetMap actually
    - teams that used the tool w/ visual cues are more likely to succeed in accomplishing the task
    - visual cues also encourage participants to engage more in the discussion + group work

\textcolor{red}{more on what techniques/design attributes folks use; talk about how to use visuals to help make sense of long linear information in a more digestible way (dialogue mapping)}

An array of previous work has supported the notion that visual aids in conversation can reduce cognitive load \textcolor{blue}{and increase group performanace in accomplishing tasks as a team.}
\cite{gumiennySupportingSynthesisInformation2014} found that participants appreciated both the visualization of sequential information as well as the flexibility to cluster certain pieces of information together as necessary, and that participants as a whole appreciated the ability to visually highlight the most relevant portions of the conversation.
\cite{HowDisplayGroup} found that visualizating conversational content through clustered nodes improved memorability of the information \textcolor{blue}{which aligns with \cite{kirshenbaum2021traces}'s finding that information stored in some sort of visual format can reduce cognitive load}.

Both real-time analysis and feedback as well as a structured visual representation of the conversation frequently have a direct, positive impact on participants' behaviors without significantly increasing their cognitive loads \cite{leshedVisualizingRealtimeLanguagebased2009}, \cite{yangCatchLiveRealtimeSummarization2022}, \cite{khadpeEmpathospherePromotingConstructive2022}, \cite{tangConceptGuideSupportingOnline2021}. Visualizing a conversation's content in a structured manner can also lead to more creativity in the discussion \cite{valkIdeationCompassSupporting2022}, as well as help with quick and efficient understanding of the team's status relative to project progress \cite{wangCallistoCapturingWhy2020}.  

\cite{tangConceptGuideSupportingOnline2021} -- tool that does concept-map based recommendation; demos the pro of visualization
    - one big takeaway: selective visuals --> eases cognitive load
\cite{wangCallistoCapturingWhy2020} -- tool that captures decision-making process in data scientists' meetings
    - big idea is that capturing the links between (a) code in computational notebooks (b) and utterances from discussion is helpful
    - the relationship visualization significantly helps w/ newcomer understanding of what's going on

\textcolor{red}{notation schema to support note-taking in meetings}
\textcolor{red}{what is the relative merits and downsides of having people take notes themsleves versus have a note-taker take notes for them? }
\textcolor{red}{from xu: i think there's research suggesting note-taking verbatimly takes away people's cognitive capacity in understanding, maybe you can cite that to.}

\cite{leshedVisualizingRealtimeLanguagebased2009} -- similar to above, it introduces the tool used (GroupMeter); found that real time *visual* feedback + linguistic analysis can lead to behavior changes
    - both dynamic (real-time) and historical views were useful to participants and affected their behavior in the meeting; both > no visuals
    - feedback from tool caused increase in reflection on language use
    - they find that visualization doesn't increase cognitive load
    - feedback also increased agreement, decreased disagreement when seeing analysis of their live dialogue 
\cite{valkIdeationCompassSupporting2022} -- tool that does live topic modeling and visuals, shows an increase in performance
    - currently a lack of CSTs (creativity support tools) that provide visuals
    - basically the tool does topic modeling (LDA) live and shows visuals to users
    - cool; visuals helped remind users to stay on topic + inspired different conversation directions (so encouraged creativity)
\cite{yangCatchLiveRealtimeSummarization2022} -- tool to do real time video stream summarization; can be used as an exmaple of AI for sensemaking 
    - again not really AI
    - tool that provides real-time summary of video content + user interaction
    - their aim is to aid viewers joining in middle of video; viewers note that what's important to them is (1) getting varying levels of detail for content up to join-point (2) catching up w minimal interruption to their attention to current stream 
    - the tool just segments the video and uses highlight content to 'summarize' those segments
    - timeline view is helpful 
    - open research direction towards how to make sense of info from before they joined stream
    - users using the tool were more engaged w the video

\cite{gumiennySupportingSynthesisInformation2014} -- tool for whiteboarding ideas as individuals and as team in mtg
    - participants want to be able to highlight / visualize bits of information that are most important
    - evidence that a 'mixed' set of visuals (i.e. mix between sequential and more flexible info or ability to move around info) is good to cater to different individuals' preferences
    - clustering of information is a helpful visual
\cite{hindalongAbstractionsVisualizingPreferences2022} -- lit review on tools for visualizing group decision making
\cite{HowDisplayGroup} -- group information in nodes, visualization, helps memorability
\cite{kontogiorgosGroundingBehavioursConversational2021} -- i don't fully get it but gist is that interface will affect how ppl are able to collaborate / participate in mtg
\cite{liuConsensUsSupportingMultiCriteria2018} -- visualizing disagreemtns leads to better alignment between participants
\cite{mackenzieWisdomDecisionSupport2006} -- decision-making supplementary tool design approach for 'wicked' problems
\cite{sunHowStudentsGenerate2022} -- case study w/ elementary school students, mind-mapping is shown to be an effective strategy in group brainstorm

\subsection{Using AI to Support Meeting Sensemaking}

AI has demonstrated utility in supporting sensemaking in meetings. AI tools that provide participants with real-time feedback in the conversation can directly impact the behavior of participants to better accomplish the task at hand \cite{leshedVisualizingRealtimeLanguagebased2009}. 

In recent years, LLMs have demonstrated adeptness at a wide variety of NLP tasks associated with dialogue and communication, from \cite{} to \cite{}. 


\cite{ImprovingTeamworkUsing} -- real-time lanugage feedback to student group mtgs [[check how they're creating the feedback]] ** not AI 
\cite{leshedVisualizingLanguageUse2010} -- visualize linguistic analysis of conversation for building teamwork; *how to balance visuals w/ not taking up participant attention by too much* --> they propose future directions of research, nothing super concrete
\cite{khadpeEmpathospherePromotingConstructive2022} -- tool to mitigate issues in virtual meetings
    - ths is not AI, btw; basically the system is that participants in a meeting do a perspective-taking exercise where they (a) provide feedback to the system about what they feel (b) receive feedback from system about how good they are at guessing how others feel
    - the system improved team viability + team willingness to give and receive feedback
    - **this isn't hugely relevant, prob won't include this
\textcolor{red}{converting meeting content/general content into an easily digetible structure}
\cite{Jiang2023GraphologueEL} -- indirectly relevant; interface to convert long text responses from chatgpt into graph-like structure diagrams for easier sense-making
    - use GPT-4 to construct graph represnetations of dialogue using node-links
    - GPT-4 is instructed to segment and annotate entities as nodes and their relationships
    - good performance by GPT on the annotation task
    - participants find that node-link diagram helps fast + easy comprehension
    - again participants enjoy having multiple visual representations (i.e. node-links, original text, outline) 
\cite{kangSynergiMixedInitiativeSystem2023} -- tool that uses LLMs to synthesize scholarly texts in a readable, graph(?) way
    - pipeline: user highlights text, loopy belief propagation algo creates a graph out of the highlights, important papers from graph used as input to GPT which extracts highlights and summarizes + structures hierarchically; finally user is able to modify the final structure if they want
    - results --> tool provides high quality outlines for participants
        - again (sim to other tools reviewed) the visualization + tool results in higher participation + engagement from participants
    - note about the tradeoff between complete info + info overload; need a way to better trim down the info visualized, but generally participants found that it eased their cognitive load to focus on broader-picture items and relationships
\cite{kimCellsGeneratorsLenses2023} -- framework for using LLMs to aid in 'object oriented interaction'
    - **this has some good notes to consider re: framework for using LLMs thru interface but idk if nec to cite directly 
\cite{kimSystematicReviewDyadic2021} -- lit review of visualizing conversation structure
    - just provides a review of systems, not really insightful
\cite{Suh2023SensecapeEM} -- interface for working w/ LLMs to get info in a more natural, not nec linear way


\textcolor{red}{generally more AI help in meeting stuff}
\cite{gonzalezAutomaticallyGeneratedSummaries2023} -- adding a gpt generated video summary to lecture increased exam performance in students who used the summary
    - nothing too complex, literally just what is mentioned above
\cite{kimModeratorChatbotDeliberative2021} -- chatbot that provides structure + semi-supervises a discussion
    - related work discusses how arguments can only be reasonable/logical if they're based in conversation up until to that point and also if they're actually logically sound --> can make the point that it's crucial then for participants to be on the same page about what's transpired in the conversation
    - results: adding structure to the discussion improves quality 



\cite{Jiang2023Graphologue}
\cite{leePromptiverseScalableGeneration2022} -- prompt generation method; prompt == query for video / info in a video that will help that specific learner; they use knowledge graphs in pipeline
\cite{liSupportingDynamicSituation2013} -- very similar to meetmap i think
    - discussion on the importance of situational awareness (a few levels that reflect participant understanding of what has happened and what will happen) --> paper explores how visuals can help w/ SA 
    - this is basically MeetMap, the visual is just a 'neighborhood' of regions of topics rather than graphical interface w nodes
    - takeaway is that users should work w/ system to develop nice visual 



\cite{Jansen2017AnIR} -- lit review on cognitive load in meetings
    - ORGANIZED + STRUCTURED content improves note-taking + memorability
    - computer note-taking generally better, thought due to speed + ability to focus more attention on incoming info

\cite{costley2021collaborative} -- study of collaborative note-taking and effects on cognitive load + group performance
    - main takeaway: collaborative note-taking pros of content understanding outweight cons of possible confusion, and doesn't overwhelm cognitive load

\cite{}
